End-to-End Far-Field Speech Recognition with Unified Dereverberation and Beamforming

Despite successful applications of end-to-end approaches in multi-channel speech recognition, the performance still degrades severely when the speech is corrupted by reverberation. In this paper, we integrate the dereverberation module into the end-to-end multi-channel speech recognition system and explore two different frontend architectures. First, a multi-source mask-based weighted prediction error (WPE) module is incorporated in the frontend for dereverberation. Second, another novel frontend architecture is proposed, which extends the weighted power minimization distortionless response (WPD) convolutional beamformer to perform simultaneous separation and dereverberation. We derive a new formulation from the original WPD, which can handle multi-source input, and replace eigenvalue decomposition with the matrix inverse operation to make the back-propagation algorithm more stable. The above two architectures are optimized in a fully end-to-end manner, only using the speech recognition criterion. Experiments on both spatialized wsj1-2mix corpus and REVERB show that our proposed model outperformed the conventional methods in reverberant scenarios.

==> acronyms.tex <==
\newacronym{asr}{ASR}{automatic speech recognition}
\newacronym{blstm}{BLSTM}{bidirectional long-short term memory}
\newacronym{blstmp}{BLSTMP}{bidirectional long-short term memory with projection}
\newacronym{casa}{CASA}{computational auditory scene analysis}
\newacronym{cer}{CER}{character error rate}
\newacronym{cirm}{cIRM}{complex ideal ratio mask}
\newacronym{cnn}{CNN}{convolutional neural network}
\newacronym{ctc}{CTC}{connectionist temporal classication}
\newacronym{dct}{DCT}{discrete cosine transform}
\newacronym{dft}{DFT}{discrete {Fourier} transform}
\newacronym{dnn}{DNN}{deep neural network}
\newacronym{doa}{DOA}{direction of arrival}
\newacronym{dpcl}{DPCL}{deep clustering}
\newacronym{e2e}{E2E}{end-to-end}
\newacronym{fft}{FFT}{fast {Fourier} transform}
\newacronym{gan}{GAN}{generative adversarial network}
\newacronym{gcc}{GCC}{generalized cross correlation}
\newacronym{gcc-phat}{GCC-PHAT}{generalized cross-correlation phase transform}
\newacronym{gmm}{GMM}{{Gaussian} mixture model}
\newacronym{hmm}{HMM}{hidden {Markov} model}
\newacronym{ibm}{IBM}{ideal binary mask}
\newacronym{irm}{IRM}{ideal ratio mask}
\newacronym{ipd}{IPD}{interaural phase difference}
\newacronym{lstm}{LSTM}{long-short term memory}
\newacronym{mfcc}{MFCC}{{Mel}-frequency cepstral coefficient}
\newacronym{mfccs}{MFCCs}{{Mel}-frequency cepstral coefficients}
\newacronym{mimo}{MIMO}{multi-input multi-output}
\newacronym{mlp}{MLP}{multilayer perceptron}
\newacronym{mse}{MSE}{mean square error}
\newacronym{mvdr}{MVDR}{minimum variance distortionless response}
\newacronym{mpdr}{MPDR}{minimum power distortionless response}
\newacronym{nmf}{NMF}{non-negative matrix factorization}
\newacronym{pca}{PCA}{principal component analysis}
\newacronym{pesq}{PESQ}{perceptual evaluation of speech quality}
\newacronym{pit}{PIT}{permutation invariant training}
\newacronym{plp}{PLP}{perceptual linear prediction}
\newacronym{psd}{PSD}{power spectral density}
\newacronym{relu}{ReLU}{rectified linear unit}
\newacronym{rir}{RIR}{room impulse response}
\newacronym{rirs}{RIRs}{room impulse responses}
\newacronym{rnn}{RNN}{recurrent neural network}
\newacronym{s2s}{S2S}{sequence-to-sequence}
\newacronym{sdr}{SDR}{signal-to-distortion ratio}
\newacronym{snr}{SNR}{signal-to-noise ratio}
\newacronym{srp-phat}{SRP-PHAT}{steered-response power phase transform}
\newacronym{stft}{STFT}{short-time {Fourier} transform}
\newacronym{stoi}{STOI}{short-time objective intelligibility}
\newacronym{svm}{SVM}{support vector machine}
\newacronym{tts}{TTS}{text-to-speech}
\newacronym{vad}{VAD}{voice activity detection}
\newacronym{wer}{WER}{word error rate}
\newacronym{wpe}{WPE}{weighted prediction error}
\newacronym{wpd}{WPD}{weighted power minimization distortionless response}
